Straggler-Resilient and Communication-Efficient Distributed Iterative Linear Solver

We propose a novel distributed iterative linear inverse solver method. Our method, PolyLin, has significantly lower communication cost, both in terms of number of rounds as well as number of bits, in comparison with the state of the art at the cost of higher computational complexity and storage. Our algorithm also has a built-in resilience to straggling and faulty computation nodes. We develop a natural variant of our main algorithm that trades off communication cost for computational complexity. Our method is inspired by ideas in error correcting codes.

==> intro.tex <==
Over the last decade, owing to the increasing {data} volumes, data processing is commonly done in large distributed systems.  The collective processing capacity of multiple computing nodes operating in parallel is higher, and as a consequence, distributed algorithms are significantly faster and often more memory efficient, as compared to single node computations. However, the performance of such distributed algorithms {does not scale linearly with the number of nodes (beyond a few tens of nodes)} in practice because of two major bottlenecks \cite{qi2016paleo, dean2012large}. First, the overhead of communicating data becomes significant in comparison to the actual computation time. Second, a few excessively slow nodes called \emph{stragglers} often slow down the overall computation. The {goal} of our paper is to develop new distributed algorithms for linear inverse solvers that overcome communication bottlenecks and stragglers.

Our specific focus is on iterative methods for linear inverse problems, where each iteration has the form $\mathbf{x}_{\textrm{new}} = \mathbf{A}\mathbf{x}_{\textrm{old}}+\mathbf{Q}\mathbf{y},$ where $\mathbf{y}$ is the input to the system. This method includes, as its special case, a wide array methods such as the Jacobi iterative method, Gauss Siedel method, power iterations and Pagerank \cite{atkinson2008introduction,heath2002scientific,kang2009pegasus,gleich2004fast}. Such iterative techniques are used extensively for solving linear inverse problems arising in imaging and inference, both for dense and sparse problems, because of their low complexity \cite{zhang2009cuda, atkinson2008introduction, bertero1998introduction}. A naive baseline method to implement such algorithms in a distributed network of processing nodes is to distribute $\mathbf{A}$ among the nodes, and perform the matrix-vector multiplication $\mathbf{A}\mathbf{x}_{\textrm{old}}$ in distributed manner. When performed over a set of $P$ distributed worker nodes, the per-node computational and storage complexities are both $\frac{1}{P}$ of the overall computational and storage complexities of the centralized algorithm. The main {difficulty with such} distributed implementations, however, is that each node only has a local view of vector $\mathbf{x}_{new}$, and messages need to be exchanged in \emph{every iteration} to concatenate/aggregate the outputs of all nodes before proceeding to the next iteration. 

\subsection*{Summary of Contributions}
Our main contribution is a new, non-trivial method of parallelizing iterative linear inverse solvers that requires significantly smaller communication overhead as compared with state of the art, both in terms of the number of rounds of communication and the number of bits communicated.  In addition to having smaller communication,  our algorithms have built in resilience to straggling and/or faulty computing nodes. We present our algorithms and results in a master-worker architecture, where there are one master node and $P$ worker nodes. The worker nodes, which operate in parallel, carry the computational burden of the iterative linear inverse solver.

The master node performs any necessary pre-processing of the inputs and sends them to the worker nodes. It also accumulates results of worker nodes, performs any necessary post-processing, and sends the results back to the worker nodes for the next set of iterations if necessary. For instance, in the baseline algorithm explained above, to perform $n$ iterations, $n$ rounds of communication are performed between the master and the worker node.

In Section \ref{sec:parallel-extreme1}, we develop the \emph{PolyLin} algorithm which has only \emph{one} round of communication between the master node and the worker nodes, irrespective of the number of iterations performed. {PolyLin guarantees linear convergence, that is, the error decays exponentially in the number of iterations.} The core idea of PolyLin is the development of a technique that computes the $n$-th power of $\mathbf{A}$ without requiring $n$ rounds of communication, or requiring every node to store $\mathbf{A}$ entirely. The total amount of data exchanged between the master node and each worker node is approximately twice the length of the target vector $\mathbf{x}$. In contrast, to perform $n$ iterations, the baseline scheme requires $n$ rounds of communication, and the amount of data exchanged is $2n$ times the length of the target vector $\mathbf{x}$, i.e., it scales linearly in the number of iterations. {Additionally, our algorithm has the property that it tolerates stragglers or faulty nodes, that is, in a system with $P$ processing nodes, it suffices if any $K$ of the $P$ nodes complete their job per round of communication; the per-node processing complexity and memory depends on $K$.}

Our algorithm incurs two penalties as compared to the baseline algorithm. First, {PolyLin} requires a fraction of {$\frac{1}{K^{2/n}}$} of the overall computational and storage complexity of the centralized algorithm {where $K\leq P$}; note that the baseline algorithm requires a fraction of $\frac{1}{P}$. Second, {PolyLin} incurs a pre-processing computation cost that, in effect, is equivalent to running the centralized algorithm once in each worker node. {Our experiments in Section \ref{experiment}, reveal that, despite the computational complexity overhead of our algorithms, the communication overhead reduction translates to faster completion time.}  The pre-processing depends only on linear system matrices/vectors $\mathbf{A},\mathbf{Q}$, and therefore can be amortized over multiple uses of the algorithm corresponding to different instances of the input $\mathbf{y}$. From an application viewpoint, the pre-processing cost may be worth the gains in communication and computation complexities when the matrices involved $\mathbf{A},\mathbf{Q}$ are fixed or slowly changing with respect to the target vector, e.g., inference and web queries. One specific example is the personalized PageRank problem where web queries may focus on different topics \cite{haveliwala2003topic} but the underlying linear system matrix (the graph adjacency matrix) does not change. Some other examples include supervised $\ell_2$-minimization with multi-instance learning and multi-label learning and solving numerical equations, such as Poisson equations, with the same system matrix but different inputs.


We develop a variant of {PolyLin} in Section \ref{sec:tradeoff} that trades off the number of rounds with respect to the computation and storage complexities. For instance, by choosing parameters correctly, Section \ref{sec:tradeoff} can be used to develop an algorithm that halves the communication cost as compared to the baseline distributed implementation but incurs a computational and storage complexity penalty of a factor of $\sqrt{P}$. {PolyLin} works by storing carefully constructed linear projections of the matrix $\mathbf{A}$ at each worker as a part of pre-processing. The worker nodes run an iterative algorithm based on the stored linear projections and the initialized target vector $\mathbf{x}$, and send the output to the master node. The coefficients for the linear projections are chosen to be evaluations of certain polynomials to ensure that the master node, on receiving the outputs of the worker node, can recover the solution of the iterative linear solver using polynomial interpolation. Robustness is built into the algorithm in a manner that is similar in spirit to Reed Solomon codes \cite{roth2006introduction}, where, the number of polynomial evaluations chosen is higher than the degree of the polynomial so that a few slow or faulty nodes can be ignored in the interpolation.

\subsection*{{Related Works}}


{Our} work relates to a long line of work that we review in three categories: distributed optimization, distributed linear system solvers and coding theoretic ideas for straggler resilient distributed computing.

 \textbf{1) Distributed optimization}: One can consider the linear inverse solver to be equivalent to a linear regression problem of the form \begin{align}\arg\min_x\|\mathbf{M}\mathbf{x}-\mathbf{y}\|^2_2\label{eq:optimization}.\end{align} Therefore, we compare our results with other communication-efficient distributed optimization algorithms\footnote{{As we mostly focus on square linear systems, we compare with distributed optimization in a regime where the number of data points is comparable to the number of features.}}. We have the following two cases:

{\textbf{1.1) One-shot communication schemes:} At one extreme, there are distributed methods that require only a single round communication such as \cite{mcdonald2009efficient,zinkevich2010parallelized,zhang2012communication,mcwilliams2014loco,heinze2016dual}. In these works, the data is distributed to the worker nodes, and {each worker node solves a ``local'' optimization on the part of the input stored at the worker, and the master node averages the results of the workers. As a consequence, the convergence of these one-shot algorithms is not linear; in fact, some of these algorithms can not guarantee convergence rates beyond what could be achieved if we ignore data residing on all but a single computer \cite{shamir2014communication}.} {In contrast, our one-round algorithm achieves linear convergence although with some computational and storage overhead.}%Also, there is some lower bound on the minimum number of rounds needed for a given approximate quality as presented in \cite{balcan2012distributed} and \cite{arjevani2015communication}. 

{{\textbf{1.2) Multiple-round communication schemes:}}  {In order to compare our schemes with algorithms in \cite{lee2017distributed,zhang2015disco,shamir2014communication,ma2015adding,nesterov2013introductory}, we focus on the regime where the number of data points is comparable to the number of features.} {We show that for our algorithms, when the number of iterations $n$ satisfies $n\geq \log_{\frac{1}{|\sigma_1|}}\frac{N\underset{1\leq i\leq N}{\max}|\alpha_i|}{\epsilon}$, the error is upper bounded by $\epsilon$, where $N$ is the number of data points, $\sigma_1$ is the second largest eigenvalue of $\mathbf{A}$, and $\alpha_i$ is the projection of an arbitrarily chosen initialization vector on to the $i$-th eigen vector of $\mathbf{A}$.} \cite{lee2017distributed} introduces two algorithms {\emph{distributed stochastic variance reduced gradient} (DSVRG) and \emph{distributed accelerated stochastic variance reduced gradient} (DASVRG)}. These algorithms respectively require $(1+\frac{\kappa P}{N})\log(\frac{1}{\epsilon})$ and $(1+\sqrt{\frac{\kappa P}{N}})\log(1+{\frac{\kappa P}{N}})\log(\frac{1}{\epsilon})$ rounds of communication to find the optimal solution with error $\epsilon$, where  $\kappa$ is the condition number as defined in \cite{lee2017distributed}. The corresponding computational and communication costs are $O(\frac{N^2}{P}+N\kappa)\log(\frac{1}{\epsilon})$ and $O(\frac{N^2}{P}+N\sqrt{\frac{\kappa P}{N}})\log(1+\frac{\kappa P}{N})\log(\frac{1}{\epsilon})$ respectively. Note that for the case that {$\kappa=\Omega({\frac{N}{P}})$} with $\theta>1$, our baseline algorithm outperforms DSVRG and DASVRG in terms of computational and communication cost. { While \cite{lee2017distributed} provides a lower bound of $\Omega(\sqrt{\frac{P\kappa}{N}})$ on the number of rounds of communication for a certain class of algorithms where the algorithm of our paper  storage cost is fixed to be that of the baseline algorithm\footnote{To the best of our understanding, the lower bound of \cite{lee2017distributed} requires a specific method of sampling and storing the data as well.} (in an order sense), in our paper we present an algorithm with a fewer number rounds although with a higher storage cost.} For instance, by loading higher computation task at each processing node, we can achieve linear convergence using only one round of communication.

 {Additionally, there have been several other algorithms such as Disco \cite{zhang2015disco}, Dane \cite{shamir2014communication}, COCOA$^{+}$ \cite{ma2015adding} and accelerated gradient method \cite{nesterov2013introductory}.} We compare algorithms {in \cite{lee2017distributed,zhang2015disco,shamir2014communication,ma2015adding,nesterov2013introductory,karakus2017straggler,maity2018robust}} in terms of communication and computational costs in Table \ref{table:comp} {briefly} and in more detail in the appendix. Specifically, our results imply that when $N$ is of the same scaling as $1/\epsilon$ and the number of features, our algorithm outperforms the baseline while the baseline is comparable with these algorithms in terms of communication rounds.}

{\textbf{2) Distributed linear inverse solver using network properties:}} {There is a second line of related works in \cite{demmel2008avoiding,demmel2012communication,wicky2017communication,lipshitz2012communication}
which minimizes the communication cost for various network architectures. {In contrast,} our work does not have these specific network structures. Some of these methods build upon the Krylov-subspace methods. In this work, we mainly focus on stationary methods (such as Jacobi and power iterations) which have successive matrix-vector multiplications. For the specific problem of PageRank, the convergence of Krylov methods strongly depends on the properties of the graph and is non-monotonic. Although Krylov methods have gained popularity, the techniques presented in our paper are still relevant for many specific problems and systems where power iterations perform comparably, or better than Krylov subspace method. Power-iteration and Jacobi methods have approximately the same {convergence rate} determined by the \emph{teleport} probability and the most stable convergence pattern \cite{gleich2004fast}. This is an advantage of stationary methods that perform the same amount of work per any iteration.} Extending our ideas to perform multiple iterations of non-stationary algorithms with fewer rounds of communication, without having to distribute all the data to all the nodes, is an interesting area of future work.

 {\textbf{3) Coding Theoretic approaches for straggler-resilient distributed computing:}} Our algorithms are related to and inspired by recent work that uses error correcting codes for protecting distributed linear operations and optimization problems \cite{dutta2016short, MatDot,MatDot_Allerton, raviv2017gradient, tandon2017gradient,raviv2017gradient, yang2017coding,lee2017speeding, mallick2018rateless,charles2017approximate,karakus2017straggler,ye2018communication,yu2017polynomial,yu2018straggler} from faults and stragglers. 
{Specifically, the approaches of  \cite{karakus2017straggler, tandon2017gradient, raviv2017gradient, yang2017coding, charles2017approximate, karakus2017straggler, ye2018communication} {can be} interpreted in our context as the introduction of coding methods for adding straggler/fault tolerance to the baseline algorithm. Since these papers essentially include a variant of the baseline algorithm, the communication overheads, measured in terms of number of rounds as well as the number bits, are proportional to the number iterations of the power method. The main contribution of our work to this body of literature is to develop a novel method that can perform multiple iterations of the power method in a single communication round, thereby reducing the overall communication cost (in addition to providing straggler resilience).}  


From a technical viewpoint, our core ideas are related to references \cite{yu2017polynomial, MatDot, MatDot_Allerton, yu2018straggler} which use polynomial evaluation based error correcting codes to protect matrix multiplications from faults, stragglers and errors. Our approach particularly builds on \cite{MatDot} which multiplies multiple (more than two) matrices in a straggler resilient manner. The process of adapting the ideas of \cite{MatDot} to the power method however requires the development of new ancilliary results; the relevent ideas of \cite{MatDot} as well as some new related results are described in Sec. \ref{sec:Propertiesofmatrixpoly}.



%Although the Krylov methods have the highest average convergence rate and fastest convergence by the number of iterations, on some graphs, the actual runtime can be longer than the run time of simple Power iterations. 

